Verification of a Generative Separation Kernel

We present a formal verification of the functional correctness of the Muen Separation Kernel. Muen is representative of the class of modern separation kernels that leverage hardware virtualization support, and are generative in nature in that they generate a specialized kernel for each system configuration. These features pose substantial challenges to existing verification techniques. We propose a verification framework called conditional parametric refinement which allows us to formally reason about generative systems. We use this framework to carry out a conditional refinement-based proof of correctness of the Muen kernel generator. Our analysis of several system configurations shows that our technique is effective in producing mechanized proofs of correctness, and also in identifying issues that may compromise the separation property.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	main.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> ccs-body.tex <==
\section{Introduction}

This is a sample!  It does not have a lot of fancy stuff in it, but if
you want to see a more complex sample, look at the original ACM
templates.

To fill up enough text to fill up 3 pages, we've included the CCS Call
for Papers three times.  It is always a good idea to include some
gratuitious citations to recent CCS papers~\cite{medvinsky1993netcash,
  bellare1993random, anderson1993cryptosystems, blaze1993cryptographic}.

\input{cfp}
\input{cfp}
\input{cfp}

\section{Conclusions}

In conclusion, it is rarely a good idea to include the same section three times in a paper, or to have a conclusion that does not conclude.

\appendix

\section{Location}

Note that in the new ACM style, the Appendices come before the References.

\input{cfp}

\begin{acks}
% TODO: For the submission, don't include acknowledgments since they would most likely deanonymize you.
\end{acks}


==> condition-checking-v2.tex <==
\section{Checking Condition $R$}
\label{sec:condition-checking}
We now describe how to efficiently check that for a given
policy $C$, the parameters generated by Muen and those of the abstract 
specification, satisfy the condition $R$.
%
%\section{$R_1$}
%\section{Algorithms For Checking $R$}
%In 64-bit mode, Intel machine allows an address space of $2^48$ addresses.
%The injectivity property, permission match and validity check 
%have to be done for each of these addresses.
Let $N_s$ be the number of subjects.
Let $N_v$ be the maximum size of the virtual address
space, and $N_u$ the actual \emph{used} space 
which is the total size of the virtual memory components of a subject, for a subject.
$N_v$ is typically of the order $2^{48}$ bytes (approx 256TB) while $N_u$ is of the
order of 1.5GB.
Let $P$ denote the size of a paging structure in bytes, which is
of the order of 500K.
A naive way to check the conditions $R_1$ (injectivity), $R_2$ (permission-checking), 
$R_3$ (validity), and $R_4$ (content-matching), would be to use a bit
array for physical memory and iterate over \emph{all} virtual
addresses to check these conditions.
However, this runs in time proportional to $N_v$, and such an
algorithm would take days to run.
In contrast, we give a way to check these properties in time proportional to
$N_u$ for each subject. These algorithms run in a few seconds.
%%We give the idea of the algo here and the details in App.~\ref{app:checking-algos}.

To check these properties efficiently we exploit the following facts
\begin{itemize}
	\item A policy specifies memory in terms of memory components 
				which are blocks of contiguous pages.
	\item Muen generates an intermediate representation of
				physical memory (called the ``B-policy'') 
				which contains the list of all memory components 
				which have to be placed in the physical memory.
				We call this list PMemComponents. 
				Each physical memory component is specified 
				with a name called ``physical name'', size, and 
				the physical address where it has to be placed in the physical memory.
				The B-policy also contains the list of virtual memory components 
				for each subject which actually are mapped to physical memory components.
				The list of virtual memory components for a subject $s$ 
				is denoted by VMemComponents($s$).
				With each virtual memory component in a subject, 
				its name called ``logical name'', 
				logical address which is the address in the subject's virtual memory,
				the permissions of the subject,
				and the physical name of the physical memory component 
				to which it is mapped to are specified.
%				In the physical memory layout generated by Muen, 
%				these memory components are also placed as blocks of contiguous physical frames.
	\item The sum of size of all the memory components is usually much less than the physical address space
        i.e. $N_u$ is small in comparison to $N_v$.
%				In other words, a lot of virtual memory is unused and there are gaps between the memory components.
\end{itemize}
% what do we exploit

% how do we do these checks
\paragraph{Injectivity-check $R_1$} 
Checking the injectivity property of the page tables 
naively will require us to check 
for all pairs of distinct logical addresses 
possibly in two different subjects' address spaces
whether they are mapped to the same physical address 
via the corresponding page tables.
The running time of this naive check will be proportional to $N_v$
where $N_v$ is approximately 256T.
%Exploiting the facts mentioned earlier 
%we propose an algorithm whose running time is proportional to $N_c^2N_s^2$. %check this.
%$N_c$ is the maximum of VMemComponent(s) across subjects.
%$N_s$ is the number of subjects.

Since the memory components are blocks of contiguous pages and contiguous frames 
in virtual and physical address space respectively, 
checking the injectivity property reduces to checking 
whether any two memory components across subjects overlap (actually coincide) in physical memory.
We first check that the memory components in PMemComponents have been laid out
disjointly in the physical memory layout given in the B-policy, by checking for overlap.
Next we check whether the physical memory components 
corresponding to any pair of virtual memory components 
possibly from different subjects are overlapping.
If such an overlap is found, to flag it as an illegal sharing 
we also need to check whether 
one of them is not specified as a channel in the original policy and
one of them is writable. We check that one of them is writable because 
Muen allows sharing of read-only components to reduce the physical memory footprint.
Finally we check whether the page tables are generated according to the
layout in the B-policy. 
For this purpose we translate the virtual address of each page 
in every virtual memory component of each subject and 
check that it matches with the physical address calculated via the B-policy.
This algorithm assumes that $R_3$ holds (validity-check passes) because 
we have not checked this property for invalid addresses 
(logical addresses outside the memory components)
in subjects' virtual address spaces.

\begin{algorithm}[t]
	\begin{algorithmic}[1]
		\ForAll{$A$, $B$ in PMemComponents}
			\If{$ A.\PA  \leq B.\PA $}
				\If{$ A.\PA + A.Size  \geq \ B.\PA $}
					\State Output(\enquote{Illegal sharing detected.});
				\EndIf
			\EndIf	
		\EndFor
	\end{algorithmic}
	\caption{Algorithm to check overlap of physical memory components}
	\label{alg:overlap-physical}
\end{algorithm}

\begin{algorithm}[t]
	\begin{algorithmic}[1]
		\State $\mathcal{M} = \bigcup_{subject\ s} $VMemComponents($s$)
		\ForAll{$A$, $B$ in $\mathcal{M}$}
			\If{$A.\PA \leq B.\PA$}
				\If{$ A.\PA + A.Size  \geq \ B.\PA $}
					\If{$\neg\ (isChannel(A) \land isChannel(B))$} % modify the if-condition
						\If{$isWritable(A) \lor isWritable(B)$} % improve the if-condition
							\State Output(\enquote{Illegal sharing detected.});
						\EndIf
					\EndIf
				\EndIf
			\EndIf
		\EndFor
	\end{algorithmic}
	\caption{Algorithm to check overlap of virtual memory components in physical memory}
	\label{alg:overlap-virtual}
\end{algorithm}

The algorithm to check the overlapping of
two physical memory components in the physical memory layout
is shown in Algorithm~\ref{alg:overlap-physical}.
The algorithm to check the overlapping of physical memory components 
corresponding to any two virtual memory components 
is shown in Algorithm~\ref{alg:overlap-virtual}.
Finally the algorithm to check whether page tables are generated 
according to the layout in the B-policy is shown in Algorithm~\ref{alg:pt-check}.
$A.\LA$ and $A.\PA$ denote the logical address of the memory component $A$ and 
the physical address corresponding to
the logical address of the memory component $A$ respectively.
$A{.}Size$ is the size of the memory component $A$ as given in the B-policy.
In Algorithm~\ref{alg:pt-check} $p.\LA$ and $p.\PA$
denote the logical and physical address of a page $p$ respectively 
as mentioned in the B-policy.

\begin{algorithm}[t]
	\begin{algorithmic}[1]
		\ForAll{$s$ in subjects}
			\ForAll{$A$ in VMemComponents($s$)}
				\State $\page.\LA$ = $A.\LA$; \ \ // logical address
				% \State $\page . \psize$ = $m . \psize$;
				\State $\page . \PA$ = $A . \PA$; \ \ // physical address
				\While{$\page . \LA < A . \LA + A . \psize$}
					\If{$\pt_s(\page . \LA) \neq \page . \PA$}
						\State Output(\enquote{Address mismatch});
					\EndIf
					\State $\page . \LA = \page . \LA + page\_size$;
					\State $\page . \PA = \page . \PA + page\_size$;
				\EndWhile
			\EndFor
		\EndFor
	\end{algorithmic}
	\caption{Algorithm to check whether page tables are generated according to B-policy}
	\label{alg:pt-check}
\end{algorithm}

\paragraph{Permission-check $R_2$} 
Again a naive algorithm to check $R_2$ will check permission for each page
in the corresponding paging structure for each subject and 
match it with the permission given in the policy.
The running time of this algorithm will be of the order $N_sN_v$.
To check $R_2$ efficiently, 
for each virtual memory component in every subject
we check that the permission of the pages in the virtual memory component 
are set according to the permissions mentioned in the B-policy.
Again this check is dependent on the validity-check as 
we do not check the permissions for invalid addresses.
%The running time of this algorithm is $N_sN_c\times maxsize$. %find a better way to write this.
%% Algorithm~\ref{alg:permission} shows the algorithm we used to check $R_2$.
%% The logical and physical address of a page $p$ are denoted by 
%% $p.\LA$ and $p.\PA$ respectively.
%% For a virtual memory component $A$ in the subject $s$, 
%% $A.\rwe$ denotes the permission of the subject $s$ as given in the B-policy.
%% Here $\rwe_s(a)$ is a function to check read/write/exec
%% permissions of the address $a$ in the page table of subject $s$.

%% \begin{algorithm}
%% 	\begin{algorithmic}[1]
%% 		\ForAll{$s$ in subjects}
%% 			\ForAll{$A$ in VMemComponents($s$)}
%% 				\State $\page.\LA$ = $A.\LA$; \ \ // logical address
%% 				% \State $\page . \psize$ = $m . \psize$;
%% 				\State $\page . \PA$ = $A . \PA$; \ \ // physical address
%% 				\While{$\page . \LA < A . \LA + A . \psize$}
%% 					\If{$\rwe_s(\page.\LA) \neq A.\rwe$}
%% 						\State Output(\enquote{Rd/Write/Exec mismatch.});
%% 					\EndIf
%% 					\State $\page . \LA = \page . \LA + page\_size$;
%% 					\State $\page . \PA = \page . \PA + page\_size$;
%% 				\EndWhile
%% 			\EndFor
%% 		\EndFor
%% 	\end{algorithmic}
%% 	\caption{Permission checking algorithm}
%% 	\label{alg:permission}
%% \end{algorithm}


\paragraph{Validity-check $R_3$}
%To check that for each subject no invalid virtual address is mapped to a physical address
In 64-bit Intel machines, % four levels of paging are 
% used to translate a virtual address to a physical address.
%as shown in Fig.~\ref{fig:page-table-file} (a).
% That is, 
translation of each valid virtual address has to go through four paging structures
called Page Map Level 4 (PML4), page directory pointer table (PDPT),
page directory (PD) and page table (PT).
Each paging structure is an array of 512 64-bit entries.
Each entry in every paging structure contains 
the 4KB aligned address of the next level paging structure 
and few bits for other uses. 
One of these bits is called ``present'' bit which when set 
means that there is a next level paging structure for the given entry.
The translation of a given valid virtual address to a physical address uses
one entry from each level of the paging structures.
% For example as shown in Fig.~\ref{fig:page-table-file} (a),
% for the translation of the given virtual address entries x, y, z and w are used from 
% the PML4, PDPT, PD and PT paging structures respectively.
Thus if it is found while translating a given virtual address that 
the present bit is not set in one of the entries used for translation, 
it means that this virtual address is invalid.
%% For example an entry in the PML4 paging structure
%% contains the base address of one of the PDPT paging structues 
%% if the present bit in the entry is set.
To make a virtual address in a subject's address space invalid, 
Muen sets the present bit in one of the entries
used for its translation to 0 while generating the page table for the subject.

Therefore to check that only valid addresses are mapped by the page tables,
a naive way will be to translate each virtual address in each subject and 
check that only for valid virtual addresses
present bit is set in the paging structures.
The running time of this algorithm will be proportional to $N_v$ 
which is huge and it will take days to run.

Alternatively, to check $R_3$ efficiently we use the files 
which store the paging structures for all the subjects generated by Muen.
The idea is to check that the present bit is set only in the entries 
which are used for translation of valid virtual addresses.
First we describe the structure of this file and then 
we shall discuss the algorithm to check $R_3$.

Muen generates a file per subject to store the page tables based on the B-policy.
Paging structures for a subject
(PT, PD, PDPT and PML4)
are stored in this file as a contiguous sequence of 64-bit words.
%% Each 64-bit word is an entry in a paging structure 
%% which contains the address of the next paging structure 
%% (physical address of a frame in case of PT), bits for permissions, present bit, etc.
% We show the structure of the file storing the paging structures 
% in Fig.~\ref{fig:page-table-file}(b).
%
%% \begin{figure}
%% 	\begin{minipage}{\textwidth}
%% 		\centering
%% 		\includegraphics[clip, scale=0.52, trim=30 270 238 85]{address_translation.pdf}
%% 	\end{minipage}\\
%% 	\begin{minipage}{\textwidth}
%% 		\begin{center}
%% 			\begin{small}
%% 				(a)
%% 			\end{small}
%% 		\end{center}
%% 	\end{minipage}
%% 	\begin{minipage}{\textwidth}
%% 		\centering
%% 		\includegraphics[clip, scale=0.5, trim=200 100 150 50]{PageTableStructure.pdf}
%% 	\end{minipage}\\
%% 	\begin{minipage}{\textwidth}
%% 		\begin{center}
%% 			\begin{small}
%% 				(b)
%% 			\end{small}
%% 		\end{center}
%% 	\end{minipage}
%% 	\caption{(a) Address translation in Intel x86 machine. 
%% 						(b) Structure of the file storing page tables.}
%% 	\label{fig:page-table-file}
%% \end{figure}
%
In this file, 
in the beginning the entries of the PML4 paging structure are stored 
which are followed by the entries of the PDPT paging structures.
Then the entries of the PDPT paging structures are followed by 
all the entries of the PD paging structures and 
finally the entries of the PT paging structures are stored.
% In Fig.~\ref{fig:page-table-file}(a) S1, S2, S3 and S4 are 
% the sizes of each of the paging structures in the file storing the paging structures.
% In Fig.~\ref{fig:page-table-file}(b) K1, K2, K3 and K4 are the offsets in the file 
% for PML4, PDPT, PD and PT entries which are used 
% when a virtual address is translated.



To check $R_3$ efficiently, we observe that the translation of a valid virtual
address makes use of certain entries of the paging structures
in the file containing the paging structures. 
The present-bits in \emph{only} these entries should be set, and all
others should be unset.
To check this we use arrays $\PTBitArray_s$ of bits, one for each
64-bit entry in the file containing the paging structures for the subject $s$.
We translate each valid virtual address, and set the bits in the
array $\PTBitArray_s$ that correspond to each paging structure entry accessed in
the translation.
After translating all valid addresses of the subject,
we check that there is no entry in the paging structure with the
present-bit set but associated array bit unset. This is
shown in Algorithm~\ref{alg:validity}.
%MAXSIZE denotes the highest physical address assigned in the B-policy.
%This can be calculated by 
%finding the memory component which has the highest physical address,
%and then adding size of the memory component to the physical address.
%% In the algorithm, first we translate each valid virtual address for each subject $s$
%% and mark the bits in $\PTBitArray_s$ corresponding to the entries
%% which are used for the translation of the virtual address.
%% Then we check if any other entries than the ones for which the bits were 
%% marked in previous step are set.
%% If we find any such entry, this means that an invalid address is mapped to a physical address.
In Algorithm~\ref{alg:validity} $PTFile_s$ is the file containing paging structures for subject $s$.
The function Entries($PTFile_s$) returns the set of entries available in the file $PTFile_s$.
The function TestPresentBit($i$) checks whether present bit is set in the entry $i$.
We note that this algorithm runs in time $O(N_u+P)$ for each subject.


\begin{algorithm}
	\begin{algorithmic}[1]
		\State Create a Boolean array $\PTBitArray_s$ for each subject $s$
		\ForAll{$s$ in subjects}
			\ForAll{$A$ in VMemComponents($s$)}
				\State //Marking the bits in $\PTBitArray_s$ corresponding to the entries used for translation of valid virtual addresses
				\ForAll {pages $p$ in $A$}
					\State   setBit($\PTBitArray_s$, PML4\_offset) 
					\State   setBit($\PTBitArray_s$, PDPTE\_offset)
					\State   setBit($\PTBitArray_s$, PDE\_offset)
					\State   setBit($\PTBitArray_s$, PTE\_offset)
				\EndFor
			\EndFor
			\State //Checking present bit is set in any other entries
			\ForAll {$i$ in Entries($PTFile_s$)}
				\If{(TestPresentBit($i$) $= 1$) $\land$  ($\PTBitArray_s[i]$ = 0)}
					\State Output(\enquote{Invalid Page Table Entry $i$})
				\EndIf
			\EndFor
%% 			\For{($x = 0$; $x <$ PTSize($s$); $x++$)}
%% 				\If{(PagetableEntry($s,x$) $\neq 0$) and \\
%% 					\hskip4.5em (TestBit(\PTBitArray, $x$) = 0)}
%% 					\State Print (``Invalid Page Table Entry at $x$'')
%% 				\EndIf
%% 			\EndFor
		\EndFor
	\end{algorithmic}
	\caption{Validity checking algorithm}
	\label{alg:validity}
\end{algorithm}



\paragraph{Content-matching $R_4$} 
Condition $R_4$ (initial memory contents) is straightforward to
check.
We simply compare the content of the image generated by Muen with
each individual component's content (which is a specified file or
``fill'' element) byte by byte.
%Algorithm shown in Algorithm~\ref{alg:content} checks the condition $R_4$.
%
%\begin{algorithm}
%	\begin{algorithmic}[1]
%		\ForAll{$e$ in FileElements}
%			\State Seek(muenImage, $e . PhysAddr-lowestPhysAddr$)
%			\State Open($e . file$)
%			\State Seek($e . file, e . offset$)
%			\For{(\ j = 0\ ; j $<$ size($e . file$)\ ; j++)}
%				\If{fgetc($e . file$) $\neq$ fgetc(muenImage)}
%					\State Output(\enquote{Data mismatch found.})
%				\EndIf
%			\EndFor
%			\For{(\ ;\ j $< e  .  size$\ ; j++)}
%				\If{fgetc(muenImage) $\neq \lq{0}\rq $}
%					\State Output(\enquote{Data mismatch found.})
%				\EndIf
%			\EndFor
%		\EndFor
%	\end{algorithmic}
%	\caption{Content matching}
%	\label{alg:content}
%\end{algorithm}

\paragraph{Structure-matching $R_5$}
Condition $R_5$ is checked by algorithmically generating
the abstract parameter data structures and ensuring that the Muen
generated ones conform to them.
%% Memory elements in the
%% memory section of the B-policy file are classified into three
%% categories: elements with the file property, elements with the fill
%% property and elements without the file or the fill property. Elements
%% with the file property associate a file name, which is to be loaded to
%% the corresponding physical location mentioned as the physical
%% address. Fill elements are with a pattern which is to be filled in the
%% corresponding physical address. We calculate the highest and the
%% lowest physical address among the file and the fill elements. Muen
%% considers elements between these the highest and the lowest addresses
%% for the final image generation. All the other elements are simply
%% discarded and are not the part of the final image.

% Algorithm \ref{image_check} shows how we
% performed byte by byte comparison.
%% \begin{algorithm}
%% \begin{algorithmic}[1]
%% \ForAll{\textit{e} in FileElements}
%% \State $Seek(muenImage,e . PhysAddr-lowestPhysAddr);$
%% \State Open($e . file$);
%% \State Seek($e . file, e . offset$);
%% \For{$j = 0; j \textless size(e . file); j++$}
%% \If{fgetc($e . file) \neq fgetc(muenImage)$}
%% \State Output(\enquote{Data mismatch found.});
%% \EndIf
%% \EndFor
%% \For{$(;j \textless e  .  size; j++)$}
%% \If{fgetc($muenImage) \neq \lq{0}\rq $}
%% \State Outuput(\enquote{Data mismatch found.});
%% \EndIf
%% \EndFor
%% \EndFor
%% \end{algorithmic}
%% \caption{Algorithm to check the correctness of generated ISO image}
%% \label{image_check}
%% \end{algorithm}

%% The check for ``fill'' elements is done similarly.
%% Here we compared patterns associated with fill-elements and
%% the corresponding data in the Muen image. Finally, we ensured that
%% locations between the highest and the lowest address,
%% which are not the part of any file or fill element, are filled with zeros.

%% \paragraph{Data Structure Check}
%% To check condition $R_4$, 
%% we checked that the templates and the other structures are filled
%% correctly by the Muen kernel generator. For this purpose we
%% manually
%% generate structures such as the scheduling plan from the policy and
%% then compared it with structures created by the generator.

\paragraph{Results.}
We implemented our algorithms above in C and Ada, using the Libxml2
library to process policy files, and
a Linux utility \texttt{xxd} to convert the
Muen image and individual files from raw format to
hexadecimal format.

We ran our tool on 16 system configs, 9 of which (D7-*,D9-*)
were available
as demo configurations from Muen.
The remaining configs (DL-*) were configured by us to mimic
% an % MLS system
a Multi-Level Security (MLS) system 
from \cite{rushbysep}.
Details of representative configs are shown % alongside.
in Table~\ref{tab:table_config}.
For each configuration the table columns show the number of subjects,
number of CPUs, the size of physical memory needed on the processor,
the ISO image size generated by the Muen toolchain, the time taken by our condition
checking tool, and finally whether the check passed or not.

We used the 3 configs D9-* (from Ver.~0.9 of Muen) as seeded
faults to test our tool. Ver.~0.9 of Muen generates \emph{implicit}
shared memory components, and this undeclared sharing was
correctly flagged by our tool.
%

The average running time on a configuration was 5.6s.
The experiments were carried out on
an Intel Core i5 machine with 4GB RAM running Ubuntu 16.04.
%% The configurations passed all our checks, except
%% the four (D9-*) configurations which failed the $R_1$ (injectivity) check.
%% We discovered that this was due to sharing of writable
%% memory components between subjects. This sharing was not declared in the policy. 
%% The system generated by Muen for
%% these configurations would thus \emph{not} be a refinement of the abstract
%% spec. This looks to be a problem with the Muen generator.
%% The details of the configurations and the results of the checks are
%% shown in Tab.~\ref{tab:table_config}.


% \begin{wrapfigure}[12]{r}{0.5\textwidth}
% \vspace{-0.6cm}
\begin{table}
\begin{center}
% \begin{scriptsize}
\begin{small}
\begin{tabular}{|l|r|r|r|r|r|c|}
    \hline
    System
    & Sub
    & CPU
    & PMem
    & Image
    & Time 
    & Check   
    \\
     & & & (MB) & (MB) & (s) & Passed \\
    \hline
        D7\_Bochs  & 8  & 4 & 527.4  & 13.8 & 3.7  & \checkmark\\
    \hline
        DL\_conf1  & 8  & 4 & 506.5 & 12.9 & 3.7 & \checkmark\\
        DL\_conf2 & 9  & 4 & 1552.7 & 15.1& 6.8 & \checkmark\\        
        DL\_conf3  & 12  & 4 & 1050.1  & 23.3 & 6.7  & \checkmark\\
        DL\_conf4  & 16  & 4 & 1571.4  & 15.1 & 9.2  & \checkmark\\
    \hline
        D9\_Bochs  & 10 & 2 & 532.9  & 16.2 & 4.9 & \ding{55}\\
        D9\_vtd     & 16 & 4 & 1057.8 & 18.4 & 5.9 & \ding{55}\\
        D9\_IntelNuc & 10 & 2 & 567.0 & 16.2 & 5.5 & \ding{55}\\         
     \hline
\end{tabular}
\end{small}
% \end{scriptsize}
\end{center}
\caption{Checking condition $R$ on different configs}
\label{tab:table_config}
\end{table}


==> condition-checking.tex <==
\section{Checking Condition $R$}
\label{sec:condition-checking}

We now describe how to efficiently check that for a given
policy $C$, the parameters generated by Muen and those of the abstract 
specification, satisfy the condition $R$.
Let $N_v$ be the maximum size of the virtual address
space, and $N_u$ the actual \emph{used} space, for a subject.
$N_v$ is typically $2^{48}$ (approx 256T) while $N_u$ is of the
order of 1.5G.
Let $P$ denote the size of a paging structure in Bytes, which is
of the order of 500K.
A naive way to check the conditions $R_1$ (injectivity) and $R_3$
(invalid virtual addresses are not mapped), would be to use a bit
array for physical memory and iterate over \emph{all} virtual
addresses, marking the bit corresponding to this mapped physical
address.
We ensure that we never mark a bit that is already marked ($R_1$)
and that we never map an invalid virtual address ($R_3$).
However, this runs in time proportional to $N_v$, and such an
algorithm would take days to run.
In contrast, we give a way to check $R_1$ in time proportional to
$N_u$ for each subject, and $R_3$ in time proportional to $N_u$
plus the size of a page table $P$.
%%We give the idea of the algo here and the details in App.~\ref{app:checking-algos}.

To check $R_1$ and $R_2$, we exploit the fact that the Muen toolchain generates an
intermediate representation of
physical memory (called the ``B-policy'') which defines the
physical address, size and the initial content of the physical memory segments
used by Muen.
We first check that these components have been laid out
\emph{disjointly} in the physical layout given in the B-policy, by
sorting them based on base address and checking for overlap.
%% For this purpose we create a linked-list of the memory components
%% with each node describing the physical-name, the physical-address
%% (base address) and the size of the chunk. Then we sort the linked-list
%% based on the base address and check for overlap.
Next we check whether the page tables are generated according to the
layout in the B-policy. For this purpose we translate each valid
physical address of a subject through its corresponding page table and
check that it matches with the address generated by the tool
chain. %, as described in Alg.~\ref{alg:page_table_generation_check}.
Algorithm~\ref{alg:page_table_generation_check} shows our algorithm for
checking conditions $R_1$ and $R_2$.

\begin{algorithm}
\begin{small}
\begin{algorithmic}[1]
	\State
	\Comment{Checking overlap of physical memory components}
	\ForAll{$A$, $B$ in PMemComponents}
		\If{$ A.\PA  \leq B.\PA $}
			\If{$ A.\PA + A.Size  \geq \ B.\PA $}
				\State Output(\enquote{Illegal sharing detected.});
			\EndIf
		\EndIf	
	\EndFor
	\State
	\Comment{Checking overlap of virtual memory components across subjects in physical memory}
	\State $\mathcal{M} = \bigcup_{\forall subject\ s} $VMemComponents($s$)
	\ForAll{$A$, $B$ in $\mathcal{M}$}
		\If{$A.\PA \leq B.\PA$}
			\If{$ A.\PA + A.Size  \geq \ B.\PA $}
				\If{$\neg\ isChannel(A) \lor \neg\ isChannel(B)$} % modify the if-condition
					\If{$isWritable(A) \lor isWritable(B)$} % improve the if-condition
						\State Output(\enquote{Illegal sharing detected.});
					\EndIf
				\EndIf
			\EndIf
		\EndIf
	\EndFor
	\State
	\Comment{Checking correctness of generated page tables and permissions}
	\ForAll{$s$ in subjects}
		\ForAll{$m$ in VmemComponents($s$)}
			\State $\page.\LA$ = $m.\LA$; \ \ // logical address
		% \State $\page . \psize$ = $m . \psize$;
			\State $\page . \PA$ = $m . \PA$; \ \ // physical address
			\State $\page . \rwe$ = $m . \rwe$; \ \ // permissions
			\While{$\page . \LA < m . \LA + m . \psize$}
				\If{$\pt_s(\page . \LA) \neq \page . \PA$}
					\State Output(\enquote{Address mismatch});
				\EndIf
				\If{$\rwe_s(\page.\LA) \neq \page.\rwe$}
					\State Output(\enquote{Rd/Write/Exec mismatch.});
				\EndIf
			%% \If{(pt\_ex(s, $\page.LA) \neq \page . ex$)}
			%% \State Outuput(\enquote{Exec mismatch found.});
			%% \EndIf
				\State $\page . \LA = \page . \LA + page\_size$;
				\State $\page . \PA = \page . \PA + page\_size$;
			\EndWhile
		\EndFor
	\EndFor
\end{algorithmic}
\end{small}
\caption{Checking injectivity of page tables and matching the permissions}
\label{alg:page_table_generation_check}
\end{algorithm}
Here $\rwe_s(a)$ is a function to check read/write/exec
permissions of the address $a$ in the page table of subject $s$.
%% We also checked the correctness of all valid kernel addresses using a similar technique. In order to detect the sharing of non-channel physical memory chunks, we create a linked-list of subjects’ memory segments and sort them according to their base physical addresses. Algorithm \ref{illegal_sharing_check} is used to detect the overlapping between the two adjacent segments A and B.

%% \begin{algorithm}
%% \begin{algorithmic}[0]
%% \If{$A{.}physicalAddress + A{.}size \geq  B{.}physicalAddress$}
%% \If{not\_part\_of\_same\_channel(A, B)}
%% \State Outuput(\enquote{Illegal sharing detected.});
%% \EndIf
%% \EndIf


%% \end{algorithmic}
%% \caption{Algorithm to check illegal sharing of memory elements}
%% \label{illegal-sharing-check}
%% \end{algorithm}

%% From the above checks, we ensure the injectivity property of the
%% page table. That is no two logical addresses are mapped to the same
%% physical address unless they have a channel between them.

%% the ``valid'' part of the permissions, we need to check for
%% \emph{each} address $a$ in the virtual address space of a subject $s$, that the
%% page table entry for $a$ in $\pt_s$ is valid iff it is valid in the
%% virtual address space (i.e. part of a legitimate memory component).
%% To do this efficiently, 
%% of size equal to the
%% number of entries across the different tables (PDPT, PD, PT)
%% in the page table.
To check $R_3$ efficiently, we observe that the translation of a valid virtual
address makes use of certain 64 bit \emph{words} in the paging structure. The
present-bits in \emph{only} these words should be set, and all
others should be unset.
To check this we use an array \PTBitArray\ of bits, one for each
64 bit word in the paging structure.
We translate each valid virtual address, and set the bits in the
array \PTBitArray\ that correspond to each word \emph{accessed} in
the translation.
After translating all valid addresses of the subject,
we check that there is no word in the paging structure with the
present-bit set but associated array bit \emph{unset}. This is
shown in Algorithm~\ref{alg:memory_gap_check}.
We note that this procedure runs in time $O(N_u+P)$.

\begin{algorithm}
\begin{small}
\begin{algorithmic}[1]
\State Find page table file size MAXSIZE; 
\State Create an Int array \PTBitArray\ of size MAXSIZE/8
\ForAll{$s$ in subjects}
\ForAll{$m$ in VmemComponents($s$)}
\ForAll {4KB pages $p$ in $m$}
\State   setBit(\PTBitArray, PML4\_offset/8)
\State   setBit(\PTBitArray, PDPTE\_offset/8)
\State   setBit(\PTBitArray, PDE\_offset/8)
\State   setBit(\PTBitArray, PTE\_offset/8)
\EndFor
\EndFor
\For{($x = 0$; $x <$ PTSize($s$); $x = x+8$)}
        \If{(PagetableEntry($s,x$) $\neq 0$) and \\
        \hskip4.5em (TestBit(\PTBitArray, $x/8$) = 0)}
        \State Print (``Invalid Page Table Entry at $x/8$'')
\EndIf
\EndFor
\State Clear \PTBitArray
\EndFor
\end{algorithmic}
\end{small}
\caption{Memory Gap Check}
\label{alg:memory_gap_check}
\end{algorithm}

% \paragraph{Muen Image Check}
Condition $R_4$ (initial memory contents) is straightforward to
check.
We simply compare the content of the image generated by Muen with
each individual component's content (which is a specified file or
``fill'' element) byte by byte.
%% The algorithm 4 shown below checks the condition R4.
%%  \begin{algorithm}
%%  \begin{scriptsize}
%%  \begin{algorithmic}[1]
%%  \ForAll{\textit{e} in FileElements}
%%  \State $Seek(muenImage,e . PhysAddr-lowestPhysAddr)$
%%  \State Open($e . file$)
%%  \State Seek($e . file, e . offset$)
%%  \For{$j = 0; j $<$ size(e . file); j++$}
%%  \If{fgetc($e . file) \neq fgetc(muenImage)$}
%%  \State Output(\enquote{Data mismatch found.})
%%  \EndIf
%%  \EndFor
%%  \For{$(;j < e  .  size; j++)$}
%%  \If{fgetc($muenImage) \neq \lq{0}\rq $}
%%  \State Output(\enquote{Data mismatch found.})
%%  \EndIf
%%  \EndFor
%%  \EndFor
%%  \end{algorithmic}
%%  \caption{Correctness of generated ISO image}
%%  \label{image_check}
%%  \end{scriptsize}
%%  \end{algorithm}

Condition $R_5$ is checked by algorithmically generating
the abstract parameter data structures and ensuring that the Muen
generated ones conform to them.
%% Memory elements in the
%% memory section of the B-policy file are classified into three
%% categories: elements with the file property, elements with the fill
%% property and elements without the file or the fill property. Elements
%% with the file property associate a file name, which is to be loaded to
%% the corresponding physical location mentioned as the physical
%% address. Fill elements are with a pattern which is to be filled in the
%% corresponding physical address. We calculate the highest and the
%% lowest physical address among the file and the fill elements. Muen
%% considers elements between these the highest and the lowest addresses
%% for the final image generation. All the other elements are simply
%% discarded and are not the part of the final image.

% Algorithm \ref{image_check} shows how we
% performed byte by byte comparison.
%% \begin{algorithm}
%% \begin{algorithmic}[1]
%% \ForAll{\textit{e} in FileElements}
%% \State $Seek(muenImage,e . PhysAddr-lowestPhysAddr);$
%% \State Open($e . file$);
%% \State Seek($e . file, e . offset$);
%% \For{$j = 0; j \textless size(e . file); j++$}
%% \If{fgetc($e . file) \neq fgetc(muenImage)$}
%% \State Output(\enquote{Data mismatch found.});
%% \EndIf
%% \EndFor
%% \For{$(;j \textless e  .  size; j++)$}
%% \If{fgetc($muenImage) \neq \lq{0}\rq $}
%% \State Outuput(\enquote{Data mismatch found.});
%% \EndIf
%% \EndFor
%% \EndFor
%% \end{algorithmic}
%% \caption{Algorithm to check the correctness of generated ISO image}
%% \label{image_check}
%% \end{algorithm}

%% The check for ``fill'' elements is done similarly.
%% Here we compared patterns associated with fill-elements and
%% the corresponding data in the Muen image. Finally, we ensured that
%% locations between the highest and the lowest address,
%% which are not the part of any file or fill element, are filled with zeros.

%% \paragraph{Data Structure Check}
%% To check condition $R_4$, 
%% we checked that the templates and the other structures are filled
%% correctly by the Muen kernel generator. For this purpose we
%% manually
%% generate structures such as the scheduling plan from the policy and
%% then compared it with structures created by the generator.

\paragraph{Results.}
We implemented our algorithms above in C and Ada, using the Libxml2
library to process policy files, and
a Linux utility \texttt{xxd} to convert the
Muen image and individual files from raw format to
hexadecimal format.

We ran our tool on 16 system configs, 9 of which (D7-*,D9-*)
were available
as demo configurations from Muen.
The remaining configs (DL-*) were configured by us to mimic
% an % MLS system
a Multi-Level Security (MLS) system 
from \cite{rushbysep}.
Details of representative configs are shown % alongside.
in Table~\ref{tab:table_config}.
For each configuration the table columns show the number of subjects,
number of CPUs, the size of physical memory needed on the processor,
the ISO image size generated by the Muen toolchain, the time taken by our condition
checking tool, and finally whether the check passed or not.

We used the 3 configs D9-* (from Ver.~0.9 of Muen) as seeded
faults to test our tool. Ver.~0.9 of Muen generates \emph{implicit}
shared memory components, and this undeclared sharing was
correctly flagged by our tool.
%

The average running time on a configuration was 5.6s.
The experiments were carried out on
an Intel Core i5 machine with 4GB RAM running Ubuntu 16.04.
%% The configurations passed all our checks, except
%% the four (D9-*) configurations which failed the $R_1$ (injectivity) check.
%% We discovered that this was due to sharing of writable
%% memory components between subjects. This sharing was not declared in the policy. 
%% The system generated by Muen for
%% these configurations would thus \emph{not} be a refinement of the abstract
%% spec. This looks to be a problem with the Muen generator.
%% The details of the configurations and the results of the checks are
%% shown in Tab.~\ref{tab:table_config}.


% \begin{wrapfigure}[12]{r}{0.5\textwidth}
% \vspace{-0.6cm}
\begin{table}
\begin{center}
% \begin{scriptsize}
\begin{small}
\begin{tabular}{|l|r|r|r|r|r|c|}
    \hline
    System
    & Sub
    & CPU
    & PMem
    & Image
    & Time 
    & Check   
    \\
     & & & (MB) & (MB) & (s) & Passed \\
    \hline
        D7\_Bochs  & 8  & 4 & 527.4  & 13.8 & 3.7  & \checkmark\\
    \hline
        DL\_conf1  & 8  & 4 & 506.5 & 12.9 & 3.7 & \checkmark\\
        DL\_conf2 & 9  & 4 & 1552.7 & 15.1& 6.8 & \checkmark\\        
        DL\_conf3  & 12  & 4 & 1050.1  & 23.3 & 6.7  & \checkmark\\
        DL\_conf4  & 16  & 4 & 1571.4  & 15.1 & 9.2  & \checkmark\\
    \hline
        D9\_Bochs  & 10 & 2 & 532.9  & 16.2 & 4.9 & \ding{55}\\
        D9\_vtd     & 16 & 4 & 1057.8 & 18.4 & 5.9 & \ding{55}\\
        D9\_IntelNuc & 10 & 2 & 567.0 & 16.2 & 5.5 & \ding{55}\\         
     \hline
\end{tabular}
\end{small}
% \end{scriptsize}
\end{center}
\caption{Checking condition $R$ on different configs}
\label{tab:table_config}
\end{table}
% \end{wrapfigure}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:



==> prelim.tex <==
\section{Preliminaries}
\label{sec:prelim}

\begin{figure}[th]
\centering
\subfigure[First]{
\begin{scriptsize}
\begin{verbatim}

1. bool S[4];
2. unsigned T[4] = {1,2,3,0};

   void init() {
     for (int i = 0; i < 4; i++)
       S[i] = 0;
   }
   
   void elem(unsigned x) {
     return (x < 4 && S[T[x]]);
   }

   void add(unsigned x) {
     if (x < 4)
        S[T[x]] = true;
   }
\end{verbatim}
\end{scriptsize}
}
\subfigure[Second]{
\begin{scriptsize}
\begin{verbatim}
 main:
 1. x := y := t := 0;
 2. spawn(t1);
 3. spawn(t2);
\end{verbatim}
\end{scriptsize}
}
\caption{Two subfigures}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> properties.tex <==
\section{Discussion}
\label{sec:properties}

